SkillSpec: Consensus-Gated Agent Skill Evolution via Representation Specialization

Natural-language skills are textual procedural memories through which large language model (LLM) agents retain reusable task knowledge without updating model weights. Existing methods typically treat skills as either static artifacts or monolithic documents optimized using aggregate validation scores as feedback. However, representing a skill as a monolithic document restricts optimization to its textual content, without explicitly modeling the structure through which procedural knowledge is retrieved and executed. We identify a key distinction between learning what knowledge to retain and determining how to organize it: textual updates should first be validated through execution evidence, after which the retained knowledge should be structured according to its procedural dependencies and retrieval requirements. To this end, we introduce SkillSpec, a two-phase framework comprising consensus-gated evolution and representation specialization. In the consensus-gated phase, complementary editing intents generate complete candidate skills. An update is committed only when paired evaluations reach consensus, requiring sufficient overall improvement and non-negative aggregate paired gain in every repeated evaluation. In the specialization phase, signals of process and redundancy sensitivity derived from the full optimization trajectory, including accepted and rejected candidates, guide the selection of a flat, graph, or hybrid representation.Across six benchmarks and three target language models, SkillSpec improves average success rate over SkillOpt by 6.89%, averaged across the three models. These results demonstrate that reliable skill evolution and representation specialization address complementary objectives: deciding what knowledge to retain and how to structure it for inference.

==> sections/figures/skillspec_a3_workflow.tex <==
\begin{tikzpicture}[
    font=\sffamily,
    >=Latex,
    box/.style={
        draw=black!85,
        line width=0.8pt,
        rounded corners=2.5pt,
        align=center,
        minimum height=12mm,
        text width=30mm,
        fill=blue!7
    },
    compact/.style={
        box,
        text width=25mm
    },
    candidate/.style={
        box,
        text width=38mm,
        fill=green!8
    },
    validation/.style={
        box,
        text width=41mm,
        fill=yellow!14
    },
    action/.style={
        box,
        text width=31mm,
        fill=purple!8
    },
    decision/.style={
        diamond,
        draw=black!85,
        line width=0.8pt,
        aspect=2.0,
        align=center,
        inner sep=1.5pt,
        text width=34mm,
        fill=orange!13
    },
    flow/.style={
        -{Latex[length=2.2mm]},
        line width=0.9pt,
        draw=black!85
    },
    feedback/.style={
        flow,
        dashed,
        draw=blue!70!black
    },
    note/.style={
        align=center,
        font=\sffamily\scriptsize,
        text=black!65
    }
]

\node[compact] (seed) {
    \textbf{Official seed skill}\\[-1pt]
    $\Phi_0$
};
\node[box, right=8mm of seed] (rollout) {
    \textbf{Roll out incumbent}\\[-1pt]
    training successes, failures,
    and trajectories
};
\node[candidate, right=8mm of rollout] (generate) {
    \textbf{Generate candidates}\\[-1pt]
    repair \quad preserve\\
    simplify \quad rewrite\\
    optional compatible combo
};
\node[box, right=8mm of generate] (screen) {
    \textbf{Paired screen}\\[-1pt]
    candidate vs.\ incumbent
    on identical task IDs
};
\node[compact, right=8mm of screen] (finalists) {
    \textbf{Select top 2}\\[-1pt]
    deterministic finalist
    ranking
};

\node[validation, below=13mm of finalists] (confirm) {
    \textbf{Confirm on 2 channels}\\[-1pt]
    independently seeded paired validation\\
    $g_k=\#(C{\checkmark},S{\times})-\#(C{\times},S{\checkmark})$
};
\node[decision, left=12mm of confirm] (gate) {
    $\sum_k g_k \ge 3$\\[-1pt]
    and $\min_k g_k \ge 0$?
};
\node[action, left=12mm of gate] (commit) {
    \textbf{Transactional commit}\\[-1pt]
    candidate becomes
    the new incumbent
};
\node[action, below=10mm of gate] (rollback) {
    \textbf{Atomic rollback}\\[-1pt]
    restore the incumbent;
    retain audit evidence
};
\node[compact, left=12mm of rollback] (next) {
    \textbf{Next round}\\[-1pt]
    refresh evidence from
    the retained incumbent
};
\node[action, right=12mm of rollback] (warm) {
    \textbf{Frozen SkillSpec-I backbone}\\[-1pt]
    verify skill, state,
    evidence, and hashes
};
\node[validation, below=11mm of warm] (telemetry) {
    \textbf{Benchmark-blind telemetry}\\[-1pt]
    estimate PSS, RSS, confidence, support\\
    from paired SkillSpec-I trajectory evidence
};
\node[decision, left=12mm of telemetry] (route) {
    \textbf{Auto representation}\\[-1pt]
    support, PSS, RSS
};
\node[validation, below=11mm of telemetry] (structured) {
    \textbf{Structured specialization}\\[-1pt]
    flat cards, graph, or hybrid\\
    four validation-gated epochs
};
\node[compact, left=12mm of structured] (test) {
    \textbf{Frozen final test}\\[-1pt]
    complete official split
};

\draw[flow] (seed) -- (rollout);
\draw[flow] (rollout) -- (generate);
\draw[flow] (generate) -- (screen);
\draw[flow] (screen) -- (finalists);
\draw[flow] (finalists) -- (confirm);
\draw[flow] (confirm) -- (gate);
\draw[flow] (gate) -- node[above, font=\scriptsize] {yes} (commit);
\draw[flow] (gate) -- node[right, font=\scriptsize] {no} (rollback);
\draw[flow] (commit) -- (next);
\draw[flow] (rollback) -- (next);
\draw[feedback] (next.west) -| node[pos=0.25, below, font=\scriptsize] {continue} (rollout.south);
\draw[flow] (next.south) |- node[pos=0.35, below, font=\scriptsize] {after round budget} (warm.west);
\draw[flow] (warm) -- (telemetry);
\draw[flow] (telemetry) -- (route);
\draw[flow] (route.south) |- (structured.west);
\draw[flow] (structured) -- (test);

\node[note, below=4mm of seed] {
    Shared official benchmark\\
    initialization
};
\node[note, below=4mm of generate] {
    Evidence-driven diversity,
    not repeated copies of one edit
};
\node[note, below=4mm of test] {
    Test tasks never participate
    in candidate selection
};

\end{tikzpicture}

